Undecidability of $D_{<:}$ and Its Decidable Fragments

Dependent Object Types (DOT) is a calculus with path dependent types, intersection types, and object self-references, which serves as the core calculus of Scala 3. Although the calculus has been proven sound, it remains open whether type checking in DOT is decidable. In this paper, we establish undecidability proofs of type checking and subtyping of $D_{<:}$, a syntactic subset of DOT. It turns out that even for $D_{<:}$, undecidability is surprisingly difficult to show, as evidenced by counterexamples for past attempts. To prove undecidability, we discover an equivalent definition of the $D_{<:}$ subtyping rules in normal form. Besides being easier to reason about, this definition makes the phenomenon of bad bounds explicit as a single inference rule. After removing this rule, we discover two decidable fragments of $D_{<:}$ subtyping and identify algorithms to decide them. We prove soundness and completeness of the algorithms with respect to the fragments, and we prove that the algorithms terminate. Our proofs are mechanized in a combination of Coq and Agda.

==> figures/algs/dint_revealing.tex <==
\begin{figure}
  \textbf{$\wedge$-Traversal}
  \begin{mathpar}
    \inferrule*[right=\infnlabel{At-Found}{dint:at:found}]
    {T \text{ is not }\wedge}
    {T \mapsto T}

    \inferrule*[right=\infnlabel{At-Left}{dint:at:left}]
    {S \mapsto S'}
    {S \wedge U \mapsto S'}

    \inferrule*[right=\infnlabel{At-Right}{dint:at:right}]
    {U \mapsto U'}
    {S \wedge U \mapsto U'}
  \end{mathpar}
  
  \revealing
  \begin{mathpar}
    \inferrule*[right=\infnlabel{Rv-Stop}{dint:rv:stop}]
    {T \text{ is not a path}}
    {\revealingdi T T[\Gamma]}

    \inferrule*[right=\infnlabel{Rv-Top}{dint:rv:top}*]
    { }
    {\revealingdi T \top [\bigcdot]}

    \inferrule*[right=\infnlabel{Rv-Bot}{dint:rv:bot}]
    {T \mapsto T_0 \\ \revealingdi[\Gamma_1]{T_0}{T_1} \\ T_1 \mapsto \bot}
    {\revealingdi[\Gamma_1 ; x : T ; \Gamma_2]{x.A}\bot[\bigcdot]}

    \inferrule*[right=\infnlabel{Rv-Bnd}{dint:rv:bnd}]
    {T \mapsto T_0 \\ \revealingdi[\Gamma_1]{T_0}{T_1} \\\\
      T_1 \mapsto \{A : S .. U\} \\ U \mapsto U_0 \\ \revealingdi[\Gamma_1']{U_0}{U'}}
    {\revealingdi[\Gamma_1 ; x : T ; \Gamma_2]{x.A}{U'}[\Gamma_1'']}
  \end{mathpar}

  \upcast / \downcast
  \begin{mathpar}
    \inferrule*[right=\infnlabel{U-Top}{dint:u:top}*]
    { }
    {\ucdi{x.A}\top[\bigcdot]}

    \inferrule*[right=\infnlabel{D-Bot}{dint:d:bot}*]
    { }
    {\dcdi{x.A}\bot[\bigcdot]}

    \inferrule*[right=\infnlabel{U-Bot}{dint:u:bot}]
    {T \mapsto T_0 \\ \revealingdi[\Gamma_1]{T_0}{T_1} \\ T_1 \mapsto \bot}
    {\ucdi[\Gamma_1 ; x : T ; \Gamma_2]{x.A}\bot[\bigcdot]}

    \inferrule*[right=\infnlabel{U-Bnd}{dint:u:bnd}]
    {T \mapsto T_0 \\ \revealingdi[\Gamma_1]{T_0}{T_1} \\ T_1 \mapsto \{A : S .. U\}}
    {\ucdi[\Gamma_1 ; x : T ; \Gamma_2]{x.A}{U}[\Gamma_1']}

    \inferrule*[right=\infnlabel{D-Top}{dint:d:top}]
    {T \mapsto T_0 \\ \revealingdi[\Gamma_1]{T_0}{T_1} \\ T_1 \mapsto \bot}
    {\dcdi[\Gamma_1 ; x : T ; \Gamma_2]{x.A}\top[\bigcdot]}

    \inferrule*[right=\infnlabel{D-Bnd}{dint:d:bnd}]
    {T \mapsto T_0 \\ \revealingdi[\Gamma_1]{T_0}{T_1} \\ T_1 \mapsto \{A : S .. U\}}
    {\dcdi[\Gamma_1 ; x : T ; \Gamma_2]{x.A}{S}[\Gamma_1']}
  \end{mathpar}

  \caption{Definition of \revealing and new definitions of \upcast and \downcast}\label{fig:dint-revealing}
\end{figure}

==> figures/algs/dint_stare_at.tex <==

\begin{figure}
  \begin{mathpar}
    \inferrule*[right=\infnlabel{SA-Top}{dint:sa:top}]
    { }
    {\stareat T \top}

    \inferrule*[right=\infnlabel{SA-Bot}{dint:sa:bot}]
    { }
    {\stareat \bot T}

    \inferrule*[right=\infnlabel{SA-Sel1}{dint:sa:sel1}]
    {\ucd[\Gamma_1]{x.A} T \\\\ \stareat[\Gamma'_1] T U}
    {\stareat{x.A} U}

    \inferrule*[right=\infnlabel{SA-Sel2}{dint:sa:sel2}]
    {\dcd[\Gamma_2]{x.A} T \\\\ \stareat S T[\Gamma'_2]}
    {\stareat S {x.A}}

    \inferrule*[right=\infnlabel{SA-VRefl}{dint:sa:vrefl}]
    { }
    {\stareat{x.A}{x.A}}

    \inferrule*[right=\infnlabel{SA-Bnd}{dint:sa:bnd}]
    {\stareatr S {S'} \\ \stareat U{U'}}
    {\stareat{\{A : S .. U\}}{\{A : S' .. U'\}}}

    \inferrule*[right=\infnlabel{SA-Fld}{dint:sa:fld}]
    {\stareat T{T'}}
    {\stareat{\{a : T\}}{\{a : T'\}}}

    \inferrule*[right=\infnlabel{SA-All}{dint:sa:all}]
    {\stareatr S {S'} \\ \stareat[\Gamma_1 ; x : S] U{U'}[\Gamma_2 ; x : S']}
    {\stareat{\forall(x : S) U}{\forall(x : S') U'}}

    \inferrule*[right=\infnlabel{SA-Left1}{dint:sa:left1}]
    {T \text{ is not an intersection} \\\\
      \stareat S T}
    {\stareat{S \wedge U}{T}}
    
    \inferrule*[right=\infnlabel{SA-Left2}{dint:sa:left2}]
    {T \text{ is not an intersection} \\\\
      \stareat U T}
    {\stareat{S \wedge U}{T}}

    \inferrule*[right=\infnlabel{SA-Right}{dint:sa:right}]
    {\stareat T S \\ \stareat T U}
    {\stareat{T}{S \wedge U}}
  \end{mathpar}

  \caption{Definition of stare-at subtyping}\label{fig:dint-stare-at}
\end{figure}


==> figures/definitions/convertible.tex <==
\begin{figure}
  \begin{mathpar}
    \inferrule*[right=\infnlabel{Cv-Sub}{mdart:cv:sub}]
    {\subtypingmd S U}
    {\convertible x S U}

    \inferrule*[right=\infnlabel{Cv-Mu}{mdart:cv:mu}]
    {\subtypingmd{\{DS_x\}}{\{DS'_x\}}}
    {\convertible{x}{\mu(z : DS_z)}{\mu(z : DS'_z)}}

    \inferrule*[right=\infnlabel{Cv-Trans}{mdart:cv:trans}]
    {\convertible x S T \\ \convertible x T U}
    {\convertible x S U}
  \end{mathpar}
  \caption{Two types are convertible w.r.t. a variable}\label{fig:convertible}
\end{figure}


==> figures/definitions/dsubsub_def.tex <==
\begin{figure}[H]
  \begin{multicols}{2}
    \begin{align*}
      x,y,z & & \pushrightbf{Variable} \\
      S, T, U ::= & & \pushrightbf{Type} \\
                  & \top & \pushright{top type} \\
                  & \bot & \pushright{bottom type} \\
                  & \{A <: U\} & \pushright{type declaration} \\
                  & x.A & \pushright{path type} \\
                  & \forall(x : S) U_x & \pushright{function}
    \end{align*}
    \textbf{Subtyping}
    \begin{mathpar}
      \inferrule*[right=\infnlabel{All}{dsubsub:all}]
      {\subtypingdss{S_2}{S_1} \\\\ \subtypingdss[\Gamma; x : S_2]{U_1}{U_2}}
      {\subtypingdss{\forall(x: S_1)U_1}{\forall(x: S_2)U_2}}
    \end{mathpar}
    
    \begin{mathpar}
      \inferrule*[right=\infnlabel{Top}{dsubsub:top}]
      { }{\subtypingdss{T}\top}

      \inferrule*[right=\infnlabel{Bot}{dsubsub:bot}]
      { }{\subtypingdss \bot T}

      \inferrule*[right=\infnlabel{Refl}{dsubsub:refl}]
      { }{\subtypingdss T T}

      \inferrule*[right=\infnlabel{Bnd}{dsubsub:bnd}]
      {\subtypingdss{U}{U'}}
      {\subtypingdss{\{ A <: U \}}{\{A <: U' \}}}
      

      \inferrule*[right=\infnlabel{Sel}{dsubsub:sel}]
      {\subtypingdss{\Gamma(x)}{\{A <: U\}}}
      {\subtypingdss{x.A}{U}}
      
      \inferrule*[right=\infnlabel{Trans}{dsubsub:trans}]
      {\subtypingdss S T \\ \subtypingdss T U}
      {\subtypingdss S U}
    \end{mathpar}
  \end{multicols}

  \caption{Definition of $\dsubsub$}\label{fig:dsubsub_def}
\end{figure}


==> figures/definitions/fsubd_def.tex <==
\begin{figure}[H]
  \begin{align*}
    T^+ ::=& \top \quad | \quad \forall X_0 <: T_0^- .. X_n <: T_n^- .\neg T^- \\
    T^- ::=& X \quad | \quad \forall X_0 .. X_n . \neg T^+
  \end{align*}
  \begin{mathpar}
    \inferrule*[right=\infnlabel{Top}{fsubd:top}]{ }{\subtypingfd X \top}

    \inferrule*[right=\infnlabel{Var}{fsubd:var}]
    {\subtypingfd{\Gamma(X)}{\forall X_0 <: T_0^- .. X_n <: T_n^- .\neg T^-}}
    {\subtypingfd X {\forall X_0 <: T_0^- .. X_n <: T_n^- .\neg T^-}}

    \inferrule*[right=\infnlabel{AllNeg}{fsubd:allneg}]
    {\subtypingfd[\Gamma; X_0 <: T_0^-; .. ;X_n <: T_n^-]{U^-}{S^+}}
    {\subtypingfd{\forall X_0 .. X_n . \neg S^+}
      {\forall X_0 <: T_0^- .. X_n <: T_n^- .\neg U^-}}
  \end{mathpar}
  \caption{Definition of $\fsub^d$ for a fixed $n \in \mathbb{N}$~\citep{fsub-undec}}\label{fig:fsubd_def}
\end{figure}


==> figures/definitions/fsubm_defs.tex <==
\begin{figure}
  \textbf{Non-normal form}
  \begin{mathpar}
    \inferrule*[right=\infnlabel{Top}{fsubm:top}]
    { }{\subtypingfm{T}\top}

    \inferrule*[right=\infnlabel{Refl}{fsubm:refl}]
    { }{\subtypingfm T T}

    \colorbox{light-gray}{
      $\inferrule*[right=\infnlabel{Tvar}{fsubm:tvar}]
      {X <: T \in \Gamma}
      {\subtypingfm X T}$
    }

    \inferrule*[right=\infnlabel{All}{fsubm:all}]
    {\subtypingfm{S'}{S} \\ \subtypingfm[\Gamma; X <: S']{U}{U'}}
    {\subtypingfm{\forall X<:S.U}{\forall X <: S' .U'}}

    \colorbox{light-gray}{
      $\inferrule*[right=\infnlabel{Trans}{fsubm:trans}]
      {\subtypingfm S T \\ \subtypingfm T U}
      {\subtypingfm S U}$
    }
  \end{mathpar}

  \textbf{Normal form}

  \begin{mathpar}
    \inferrule*[right=\infref{fsubm:top}]
    { }{\subtypingfmn{T}\top}

    \inferrule*[right=\infref{fsubm:refl}]
    { }{\subtypingfmn T T}
    
    \colorbox{light-gray}{
      $\inferrule*[right=\infnlabel{Tvar'}{fsubmnf:tvar}]
      {X <: T \in \Gamma \\ \subtypingfmn T U}
      {\subtypingfmn X U}$
    }

    \inferrule*[right=\infref{fsubm:all}]
    {\subtypingfmn{S'}{S} \\ \subtypingfmn[\Gamma; X <: S']{U}{U'}}
    {\subtypingfmn{\forall X<:S.U}{\forall X <: S' .U'}}
  \end{mathpar}

  \caption{Non-normal form and normal form of $\fsub^-$}\label{fig:fsubm_defs}
\end{figure}

==> figures/definitions/opesubc.tex <==

\begin{figure}
  \begin{mathpar}
    \inferrule*[right=\infnlabel{Opec-Nil}{mdart:opec:nil}]
    { }
    {\opesubmd{\bigcdot}[\bigcdot]}

    \inferrule*[right=\infnlabel{Opec-Drop}{mdart:opec:drop}]
    {\opesubmd{\Gamma}}
    {\opesubmd{\Gamma ; x : T}[\Gamma']}

    \inferrule*[right=\infnlabel{Opec-Keep}{mdart:opec:keep}]
    {\opesubmd{\Gamma} \\ \convertible x S U}
    {\opesubmd{\Gamma ; x : S}[\Gamma' ; x : U]}
  \end{mathpar}

  \caption{The definition of order preserving convertible environment}
  \label{fig:opesubc}
\end{figure}

==> figures/definitions/subenv.tex <==
\begin{figure}
  \begin{mathpar}
    \inferrule*[right=\infnlabel{Se-Nil}{jdot:se:nil}]
    { }
    {{\bigcdot}\preceq \bigcdot}

    \inferrule*[right=\infnlabel{Se-Cons}{jdot:se:cons}]
    {\Gamma \preceq \Gamma' \\ \subtypingjdot S U}
    {\Gamma ; x : S \preceq \Gamma' ; x : U}
  \end{mathpar}

  \caption{Definition of sub-environment}\label{fig:subenv}
\end{figure}

==> macros.tex <==
\newcommand\meta[1]{{\color{red}META: #1}}
\newcommand\direction[1]{{\color{blue}Direction: #1}}
\newcommand\JH[1]{{\color{blue}JH: #1}}


% symbols
\makeatletter
\DeclareFontFamily{OMX}{MnSymbolE}{}
\DeclareSymbolFont{MnLargeSymbols}{OMX}{MnSymbolE}{m}{n}
\SetSymbolFont{MnLargeSymbols}{bold}{OMX}{MnSymbolE}{b}{n}
\DeclareFontShape{OMX}{MnSymbolE}{m}{n}{
    <-6>  MnSymbolE5
   <6-7>  MnSymbolE6
   <7-8>  MnSymbolE7
   <8-9>  MnSymbolE8
   <9-10> MnSymbolE9
  <10-12> MnSymbolE10
  <12->   MnSymbolE12
}{}
\DeclareFontShape{OMX}{MnSymbolE}{b}{n}{
    <-6>  MnSymbolE-Bold5
   <6-7>  MnSymbolE-Bold6
   <7-8>  MnSymbolE-Bold7
   <8-9>  MnSymbolE-Bold8
   <9-10> MnSymbolE-Bold9
  <10-12> MnSymbolE-Bold10
  <12->   MnSymbolE-Bold12
}{}

\let\llangle\@undefined
\let\rrangle\@undefined
\DeclareMathDelimiter{\llangle}{\mathopen}%
                     {MnLargeSymbols}{'164}{MnLargeSymbols}{'164}
\DeclareMathDelimiter{\rrangle}{\mathclose}%
                     {MnLargeSymbols}{'171}{MnLargeSymbols}{'171}

\newcommand*\bigcdot{\mathpalette\bigcdot@{.5}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}

\makeatother

\makeatletter
\newcommand{\xRightarrow}[2][]{\ext@arrow 0359\Rightarrowfill@{#1}{#2}}
\makeatother

\newcommand\isomorph{\xrightarrow{\sim}}

\newcommand{\Uuparrow}{\;\rotatebox[origin=c]{90}{$\Rrightarrow$}\;}

% other definitions

\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}

% \newtheorem{corollary}{Corollary}
% \newtheorem{proposition}{Proposition}
% \newtheorem*{claim}{Claim}

% \newtheorem{question}{Question}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{convention}{Convention}
% \newtheorem{problem}{Problem}
% \declaretheoremstyle[bodyfont=\normalfont]{normalhead}
% \declaretheorem[style=normalhead]{convention}

\crefname{premise}{premise}{premises}

% inference rule related
\makeatletter
\def\namedlabel#1#2{\begingroup
   \def\@currentlabel{#2}%
   \label{#1}\endgroup
}
\makeatother
\newcommand{\infnlabel}[2]{#1\namedlabel{#2}{#1}}
\newcommand{\infref}[1]{\textsc{\ref{#1}}}

\newcommand{\letin}[3]{\text{let } #1 = #2 \text{ in } #3}
\newcommand{\letinas}[4]{\text{let } #1 : #2 = #3 \text{ in } #4}

\newcommand{\inttyp}[1]{\llbracket #1 \rrbracket}
\newcommand{\intctx}[1]{\llangle #1 \rrangle}

% display of inference rules
\def\MathparLineskip {\lineskiplimit=0.8em\lineskip=0.8em plus 0.2em}
%\mprset {sep=1em, vskip=0ex}

\makeatletter
\newskip \mpr@andskip \mpr@andskip 0.7em plus 0.4fil minus 0.4em
\def \mpr@and {\hskip \mpr@andskip}
\makeatother

% tikz

% \makeatletter
% \newsavebox{\measure@tikzpicture}
% \NewEnviron{scaletikzpicturetowidth}[1]{%
%   \def\tikz@width{#1}%
%   \def\tikzscale{1}\begin{lrbox}{\measure@tikzpicture}%
%   \BODY
%   \end{lrbox}%
%   \pgfmathparse{#1/\wd\measure@tikzpicture}%
%   \edef\tikzscale{\pgfmathresult}%
%   \BODY
% }
%   \makeatother

\DeclareDocumentCommand{\pointat}{ o m m o } {
  \IfNoValueTF {#1}
  {
    \IfNoValueTF {#4}
    {
      \tikz{\draw[decoration=arrows, decorate] (0,0)
        node[xshift=-7pt] {$#2$} -- (0.5,0) node[xshift=7pt] {$#3$};}
    }
    {
      \tikz{\draw[decoration=arrows, decorate] (0,0)
        node[xshift=-7pt] {$#2$} -- (0.5,0) node[xshift=#4 pt] {$#3$};}
    }
  }
  {
    \IfNoValueTF {#4}
    {
      \tikz{\draw[decoration=arrows, decorate] (0,0)
        node[xshift=-#1 pt] {$#2$} -- (0.5,0) node[xshift=7pt] {$#3$};}
    }
    {
      \tikz{\draw[decoration=arrows, decorate] (0,0)
        node[xshift=-#1 pt] {$#2$} -- (0.5,0) node[xshift=#4 pt] {$#3$};}
    }
  }
}

\crefformat{section}{\S#2#1#3}
\crefformat{subsection}{\S#2#1#3}
\crefformat{subsubsection}{\S#2#1#3}
\crefrangeformat{section}{\S\S#3#1#4 to~#5#2#6}
\crefmultiformat{section}{\S\S#2#1#3}{ and~#2#1#3}{, #2#1#3}{ and~#2#1#3}


\newcommand{\OL}[1]{\textcolor{red}{\bfseries OL: #1}}

\newcommand{\cD}{\mathcal{D}}
\newcommand{\highlight}[1]{\colorbox{light-gray}{$#1$}}

==> makefile <==
.PHONY: all clean

TARGETS::=main.pdf template.pdf
TOREMOVE::=$(shell cat .gitignore)
TEXFILES::=$(subst ./,,$(shell find . -name '*.tex'))

all:main.pdf

${TARGETS}: %.pdf: %.tex $(filter-out $(subst .pdf,.tex,${TARGETS}),${TEXFILES})
	pdflatex -shell-escape -halt-on-error $(@:.pdf=)
	bibtex $(@:.pdf=)
	pdflatex -shell-escape -halt-on-error $(@:.pdf=)
	pdflatex -shell-escape -halt-on-error $(@:.pdf=)

temp.pdf: temp.tex
	bibtex $(@:.pdf=) || true
	pdflatex -shell-escape -halt-on-error $(@:.pdf=)

FINDCMDPRE::=${foreach x, ${TOREMOVE}, -o -name '$x'}
FINDCMD::=${wordlist 2,${words ${FINDCMDPRE}},${FINDCMDPRE}}

clean:
	find . \( ${FINDCMD} \) -exec rm {} +
	find . -name '_minted*' -exec rm -r {} +

